A Cryogenic Silicon Interferometer for Gravitational-wave Detection

The detection of gravitational waves from compact binary mergers by LIGO has opened the era of gravitational wave astronomy, revealing a previously hidden side of the cosmos. To maximize the reach of the existing LIGO observatory facilities, we have designed a new instrument that will have 5 times the range of Advanced LIGO, or greater than 100 times the event rate. Observations with this new instrument will make possible dramatic steps toward understanding the physics of the nearby universe, as well as observing the universe out to cosmological distances by the detection of binary black hole coalescences. This article presents the instrument design and a quantitative analysis of the anticipated noise floor.

==> Backscatter.tex <==
\section{Scattered Light}
\label{s:BackScatter}
The sensitivity required to make gravitational wave measurements can
be expressed also as a sensitivity to optical \textit{phase} fluctuations.
The current state of the art is approximately
$10^{-11}$ radians/$\sqrt{\rm Hz}$ and is nominally limited by
quantum mechanics and the available laser power
(cf. \Cref{s:sqz}).
Practically, however, all of the high
sensitivity interferometers in the past 30 years have been limited
at some frequencies by the non-fundamental phase fluctuations due to
scattered light. This phenomenon of excess phase noise due to scattered
light has been known about for decades~\cite{Schilling:1981} but
the methods by which to combat it have been developing steadily since
then and involve the highest levels of experimental artistry in the
field of laser interferometry.

Due to imperfections in the optics, for example, a small fraction of
the laser light escapes from the main interferometer beam path. This
light then interacts with something (e.g. a piece of the vacuum system
or some other suspended optic or beam dump) and then recombines with the
circulating laser field within the
interferometer~\cite{Kip:Scatter95, Kip:Baffles1989, Sam:Scatter2012,
Stefano:Scatter, vinet1997scattered, fritschel1998high}.
The recombination may occur at virtually any point within the system:
inside of the Fabry-Perot arm cavities, at the beamsplitter, or even at
the final photodetector which records the GW strain signal. Scattered
light induced phase noise in the sensing of auxiliary degrees of
freedom can couple into the strain channel
through the relevant feedback control systems .

%It is illuminating to consider \emph{quantitatively} the amplitude of the noise for a few of these cases.


\begin{figure}
    \begin{subfigure}{0.4\textwidth}
          \includegraphics[width=\textwidth]{Figures/ETMphasemap.png}
    %\caption{Mirror Surface Phase Map}
    \end{subfigure}

    \begin{subfigure}{0.4\textwidth}
      \includegraphics[width=\textwidth]{Figures/ETMpsd.pdf}
          %\caption{Mirror Surface PSD}
    \end{subfigure}
    \caption{(left) Surface figure of an uncoated LIGO mirror (ETM07) with the
      spherical curvature and tilt subtracted. The ripple pattern at a radius
      of 3\,--\,15\,cm from the center is due to the planetary coating technique.
      (right) 1D power spectrum of surface. Also
      plotted is the RMS surface roughness integrated from high to low
      spatial frequency.}
    \label{fig:PhaseMap}
\end{figure}
 

\subsection{Case I: The Beam Tube Baffles}
% based on T1300354
The case of scattering from the multi-km beam tubes connecting the ends of the
interferometer has been studied by Whitcomb, Weiss, Thorne, and Flanagan (for LIGO)
and by Braccini, Vinet, et al. (for Virgo); see references above. Here we provide
a condensed version of their arguments so as to construct a noise budget for backscatter.
Let us assume in this case that the field scatters from the test mass surface,
reflects from a piece of multi-km long beamtube, returns to the same test mass
mirror, and then recombines into the circulating cavity mode. The resulting
phase fluctuation of the electric field will be
\begin{equation}
\delta u_{s} = \frac{4 \pi}{\lambda} x_{s}(f) \sqrt{P_s}
\end{equation}
For comparison, the field fluctuation due to mirror motion will be
\begin{equation}
\delta u_{m} = \frac{4 \pi}{\lambda} x_{m}(f) \sqrt{P_0}
\end{equation}
where $x_s$ is the motion of the beamtube in the direction of the mirror, $x_m$
is the motion of the interferometer mirror, $\lambda$ is the laser wavelength,
$P_0$ is the power stored in the arm cavity, and $P_s$ is the power which
recombines into the circulating cavity mode. Ignoring for a moment the radiation
pressure effects, we can see that the phase noise due to this type of backscatter
can be simply expressed (in units of mirror displacement) using the ratios of
the stored power and the backscattered power which recombines with the cavity mode:
\begin{equation}
x_{m}(f) = x_{s}(f) \sqrt{\frac{P_s}{2 P_0}}
\end{equation}
where the factor of 2 comes from only including phase fluctuations of the backscattered field.

So in order to estimate the $x_m$, we will have to compute $P_s$.
This can be written down by tracing the path of the beam and considering
the relevant scattering cross sections at each step~\cite{Kip:Baffles1989}:
\begin{enumerate}
\item The probability for the main beam to scatter into some angle towards a potential backscatterer.
\item The probability for that backscatterer to scatter light back towards the mirror.
\item The probability for that backscattered field to recombine into the cavity mode.
\end{enumerate}
\begin{equation}
P_s = P_0 \frac{\lambda^2}{d^2} \delta \Omega_{ms} \frac{dP}{d\Omega_{ms}} \frac{dP}{d\Omega_{bm}} \frac{dP}{d\Omega_{sm}}
\label{eq:ScatProb1}
\end{equation}
In the above equation, the scatter probability is used; this is related to the
more commonly used Bidirectional Reflectance Distribution Function (BRDF) by
$ \mathrm{BRDF}(\theta) \times cos(\theta) = dP/d\Omega$, where $\theta = 0$
corresponds to normal incidence.
The scattering in/out of the main cavity mode has time reversal symmetry,
and so the first and last probabilities in \eqref{eq:ScatProb1} are equal:
\begin{equation}
P_s = P_0 \frac{\lambda^2}{d^2} \delta \Omega_{ms}
\bigg(\frac{dP}{d\Omega_{ms}}\bigg)^2 \frac{dP}{d\Omega_{bm}}
\label{eq:ScatProb2}
\end{equation}

\begin{figure}[h]
  \centering
    \includegraphics[width=\columnwidth]{Figures/ETM_scatter.pdf}
    \caption{Schematic diagram of a LIGO interferometer mirror
      and surrounding vacuum chambers responsible for backscattered light.}
    \label{fig:ETMscat}
\end{figure}

Based on the dimensions in Figure~\ref{fig:ETMscat}, we can see that
we should consider angles of $\sim r_{\rm tube}/d_{\rm scat}$, where
$r_{\rm tube} \simeq 0.5$\,m and $d_{\rm scat} \sim$10\,--\,4000\,m
for the mirror BRDF. 
For light scattered into these angles ($\theta_{scat} = \lambda /
\lambda_{rough} \simeq$ 0.1\,--50\,mrad), 
we need to consider spatial scales on the mirror of
 (cf. Figure~\ref{fig:PhaseMap}) $\lambda_{rough} \sim $ 0.001\,--\,1\,cm.

\subsection{Case II: The Test Mass Chambers}
During the operation of the first generation of kilometer scale interferometers,
it became clear that the scattered light from the test mass mirrors was not
all concentrated into small angles (as predicted by theory for super-polished
optics). To calculate the total power scattered into wide angles, one can use the
equivalent of Fermi's 'Golden Rule' (\Cref{eq:GoldenRule}) for optical scattering.

Combining the measurement result from
\Cref{fig:PhaseMap} with \Cref{eq:GoldenRule}, we can see that the power radiated into
angles greater than 1\,degree should be
less than 0.1\,ppm. This underestimates the true number by
at least 2 orders of magnitude.

Based on cavity ringdown and resonant reflectivity tests 
(cf.~\cite{isogai2013loss}), the round trip (arm cavity)
loss in the initial LIGO interferometers ranged from
$\sim$60\,--\,140\,ppm. For two of the Advanced LIGO interferometers, the loss
is in the $\sim$80\,--\,120\,ppm range. Wide angle, \textit{in situ},
measurements (using calibrated photodetectors and CCD cameras) show
that the total loss for $\theta_{scat} \gtrsim 1\deg$ is $\sim$\,15\,ppm.
However, it is not at all clear that the angular distribution in that
range is that of a Lambertian surface. Measurements taken at angles of
$\sim$ (0.5 m)/(4000 m) $\approx 0.1$\,mrad show a large azimuthal dependence
(i.e. the BRDF is not symmetric around the beam axis).
Images, such as the one in Figure~\ref{fig:2kETMy}, 
implicate point-like structures.
Repeated cleaning of the surface using various techniques reveals a largely
unchanging pattern, implying that the points are defects in the dielectric
mirror coatings, rather than surface contaminants. Although the details of the
story are still being investigated, it seems possible that the defects
are due to artifacts of the ion beam sputtering process~\cite{reid2016development} as well as
crystal formation~\cite{Qin:ks} in the amorphous thin films during the
post-deposition annealing.

%\subsubsection{Case III: Backscatter from the Dark Port}
\subsection{Backscatter from the Dark Port}
Another location which requires much care in design is the (dark)
detection port of the interferometer. Since it is in this location
that the very small optical phase measurements are done, any small
fields at this location can be potentially troublesome.

In particular, most of the past and current interferometers have
$\sim$5\,--\,50\,mW of light going from the beamsplitter in the
direction of the GW detection photodiodes. Some of this light is
unwanted (coming from the contrast defect of the light from the two
arms) and some is there intentionally (a local oscillator field at
either the main laser frequency or offset by tens of MHz in the case
of interferometers with heterodyne readout). As with all sources of
backscatter, the fields which scatter back into the interferometer
from the dark port produce both amplitude and phase modulation.

In order to reduce the backscatter noise from the dark port to an
acceptable level, a series of measures are generally taken:
\begin{itemize}
\item an Output Mode Cleaner~\cite{Rob:2008,Tobin:DC} cavity 
  with a ring (3 or 4 mirror) cavity
  design so as to limit the scattering into the counter propagating mode.
\item high quality optics (for low scatter) in the Output Mode Cleaner.
\item a Faraday isolator between the interferometer and the output
  detection systems.
\item appropriate angling of the photodetectors so as to minimize the
  specular reflection and minimize the backscattering into the interferometer.
\end{itemize}

One promising approach would be to limit the amount of carrier light
which is transmitted by the interferometer to the dark port. The idea
of making a balanced homodyne readout~\cite{fritschel2014balanced}
utilizing a local oscillator field from an auxiliary beam is being
pursued as a future upgrade of Advanced LIGO.


%\begin{figure}[h]
%  \centering
  %  \includegraphics[width=\columnwidth]{Figures/Cheryl-2ketmy.pdf}
   % \caption[Point defects in a LIGO mirror]{Image of an initial LIGO 
    %  test mass during normal operation. The large blob near the top
     % of the image is due to a low power diagnostic beam. The 
      %'starry night' of points are believed to be due to point 
     % defects in the high reflection coating and contribute to small 
     % and large angle scattering. Photo credit: Cheryl Vorvick}
    %\label{fig:2kETMy}
%\end{figure}


%\subsubsection{Case IV: Backscatter from the Bright Port}


==> Misc.tex <==
\label{s:Misc}

\textcolor{red}{(Another Aidan bit)}

\subsection{Compensation plate material}

\subsection{Balanced Homodyne Readout}

==> Noise.tex <==
\label{s:Noise}

%\textcolor{red}{(OK we need a paragraph followed by a noise plot.)}



The relevant noises include:
\begin{itemize}
\item Quantum --- section~\ref{s:Quantum}
\item Coating Brownian and thermo-optic --- section~\ref{s:Coatings}
\item Substrate Brownian, thermo-refractive, and carrier density --- section~\ref{s:SiliconMasses}
\item Seismic --- same as aLIGO
\item Newtonian --- reference?
\item Suspension thermal --- section~\ref{s:Suspensions}
\item Residual gas --- reference?
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/BlueBird5.pdf}
  \label{fig:GWINCnoiseBudget}
  \caption{Noise projection }
\end{figure}

%\textcolor{red}{(Doesn't this plot show that we are not limited by the facility at any frequency? Except possibly by the Newtonian Gravity noise.)}


==> OldLasers.tex <==
\label{s:Lasers}
\emph{\R{Gustafson and Brooks}} \\
In Section~\ref{s:wavelength}, the motivations for operating with a \GwincVal{Blue.Laser.Wavelength_nm}\,nm laser are discussed. Here we examine what the \emph{requirements and prospects} for such a laser are.

\subsection{Noise requirements}
We discuss now the laser noise requirements including: angular beam pointing jitter, intensity fluctuations, frequency noise, polarization fluctuations and \emph{whatever else we can think of}.

\subsubsection{Jitter noise/Pointing requirements}
We begin with a description of how jitter noise couples to DARM and include a calculation of the requirement on this. The angular jitter of the laser beam can be written as a component in a $TEM_{10}$ mode and misalignment of the interferometer optics will couple this mode into the TEM00 mode and hence into the GW signal quadrature. An analysis of the jitter noise requirement (noise on $TEM_{10}$ input beam) requires an estimate of the residual misalignment of the IFO optics, the resonant conditions of the $TEM_{10}$ in the recycling cavities and the attenuation of any input jitter noise by the input optics. The jitter noise requirement for Voyager is shown  is shown in Figure \ref{fig:jitter_noise_req} and as a comparisonwe show the requirement for aLIGO. \emph{See T0900142 for aLIGO pointing requirements.}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/aLIGO_jitter_noise_req.pdf}
  \label{fig:jitter_noise_req}
  \caption{Jitter noise requirement (for aLIGO from T0900142) and for Voyager}
\end{figure}


\subsubsection{Intensity noise}
Intensity noise coupling to DARM directly and through radiation pressure moving the core optics. Derivation of intensity noise requirement. The intensity noise requirement is shown in Figure \ref{fig:RIN_noise_req}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/Voy_PSL_RIN_requirement.pdf}
  \label{fig:RIN_noise_req}
  \caption{Relative intensity noise requirement (I have doubts about the region 10 - 100Hz. Also, the HF curve is dominated by RF SB getting onto the detection PDs. I had to guess this coupling so the location of the kink is totally false right now)}
\end{figure}

\subsubsection{Frequency noise}
Short derivation of frequency noise requirement.
The frequency noise requirement is shown in Figure \ref{fig:freq_noise_req}.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/aLIGO_freq_noise.png}
  \label{fig:freq_noise_req}
  \caption{\R{remake this plot without MS Paint} Frequency noise requirement (currently aLIGO figure as placeholder)}
\end{figure}

\subsubsection{Polarization noise}

We need to do a matrix calculation that looks at $s_{pol}$ and $p_{pol}$ inputs and estimates the coupling of the input polarization noise to the output 00 signal.

A derivation of the laser beam polarization noise requirement follows. Monocrystalline Silicon is a cubic crystal thus it is optically isotropic and cannot have birefringence.  However, residual stress, dislocations and impurities can break the symmetry resulting in a small residual birefringence.  This Birefringence can play an important part in this \cite{SiliconBirefringence2016} design because it is likely to vary throughout the volume of the material. Thus any motion of the silicon substrate or the polarization of the light is likely to result in phase noise as the light propagates through the substrate. 

Reference - Birefringence Measurements on Crystalline Silicon, C. Kruger, Class. Quantum Grav. 33 (2016) 015012 (17pp)


\subsection{Auxiliary optics}

Discussion on the impact of using \GwincVal{Blue.Laser.Wavelength_nm}\,nm on Faradays, AOMs and EOMs.

\subsubsection{Isolators}
Faradays - see Florida [Aidan]

\subsubsection{Electro-optics}
Modulators - see Florida [Aidan]

Many of the electro-optical materials that work in the visible and  at 1 micron also have low optical absorption in the \GwincVal{Blue.Laser.Wavelength_nm}\,nm wavelength region.  The Table below lists several of them and their optical properties.


\begin{table}
\centering
\begin{tabular}{ |c| c| c| c| }
    \hline
     & Transmission Range [nm] & EO Coefficient & Something Else (TM) \\
    \hline
    $ADP$ & 185-1450?? & 1 & 2 \\
    $KDP$ & 176-1420?? & 1 & 2 \\
    $KTP$ & 350-4500& 1 & 2\\
    $LiNbO3$ & 0.500-5000 & 1& 2\\ 
    $LiIO3$  & 0.380-5500 & 1 &  2 \\
    $KNbO3$  & 0.450-5000 & 1 &  2 \\
    $LBO$  & 0.170-2500 & 1 &  2 \\
    $BBO$  & 0.205-3000 & 1 &  2 \\
    
\hline
\end{tabular}
\caption{Common Electro-Optical materials with low optical absorption in the \GwincVal{Blue.Laser.Wavelength_nm}\,nm region.}
\label{tab:EOM}
\end{table}



\subsection{Prospects for a Fiber Laser for Voyager}
Emission lines in Thulium doped fibers span the 1.6 - 2.05 $\mu$m wavelength band \cite{TmLasersReview}, \cite{Richardson2010} while Holmium doped fibers span the range from 1.9 - 2.1 $\mu$m \cite{HoLasersReview2014}, \cite{Richardson2010}, \cite{Nilsson2004}. This raises the prospect of sources that span this whole region \cite{HoLasersReview2014}

GW interferometers have been using diode laser pumped free space 1064\,nm lasers because of their low amplitude and frequency noise, but this wavelength is incompatible with silicon core optics.   Moreover, the higher laser power required (\GwincVal{Blue.Laser.Power}\,W) is more compatible with the capabilities of fiber lasers. 

Current  prospects for \GwincVal{Blue.Laser.Wavelength_nm}\,nm lasers are promising. Following the architecture of Advanced LIGO of using a low power and low noise master oscillator stage, mid-power amplifier stage (35W) and high-power stage (300 - 400 W).

\begin{itemize}
\item  Master oscillator stage/low power stages: Single frequency  Holmium fiber lasers have been demonstrated with 50kHz linewidth. Available up to 5W (NP Photonics). 

\item  Medium/high power stage: Holmium fiber lasers have been demonstrated at 200W (multiple longitudinal modes) (reportedly 400W). DST group in Adelaide. Injection seeding/locking high power stage is TBD. \cite{HoLasersReview2014}
\end{itemize}



\subsubsection{Fiber Lasers}

\textit{Laser Diode Pumping} of fiber lasers uses semiconductor diode laser similar to the ones used for pumping the solid state lasers described above, but restricted to high brightness, fiber-coupled devices suitable for coupling into the cladding of the fiber. Several single stripe pump lasers can be spliced in to increase the pump power making use of the large acceptance of the cladding. Alternatively, a brightness converting solid-state laser can sometimes be used if a suitable match of materials and wavelengths can be found. \textcolor{red}{Brightness converting SSL Ref}

\textit{Polarization maintaining fiber} is required for our application. While a regular fiber is cylindrically symmetric with no preferred polarization, polarization maintaining fibers have a built-in birefringence formed during the manufacture by one of several methods, including the use of stress rods, elliptical cores and so-called Panda designs. They all introduce a preferred axis for the propagation and amplification of linearly polarized light \textcolor{red}{Pol maintaining fibers Ref}.

\paragraph{Stimulated Brillouin Scattering}

The classical picture of Brillouin scattering is a photon scattered and Doppler shifted from a moving acoustic density wave. In SBS it is the interference of the forward propagating laser beam and the backwards scattered beam that forms an acoustic grating due to electrostriction in the dielectric material. In other words the forward and counter propagating fields interfere with each other to produce an electric field that distorts the material, resulting in variations in the refractive index. The pump laser continues to build the strength of this moving grating until it is strong enough to operate as a reflector of the pump, frequency shifted by the moving grating. Threshold for SBS occurs for a pump intensity, $I (W/cm^2)$ and SBS gain length product, $g_0l$ ($g_0$ in cm/W) of $Ig_0l\sim 25$ \textcolor{red}{Zeldovich 1985 Ref}  with a more refined calculation for optical fibers finding that the threshold gain-length product for SBS depends on the fiber length and varies from about 25 for short fibers to less than 5 for very long fibers \textcolor{red}{Kovalev 2007 Ref}. For a single frequency, long coherence length laser this corresponds to a laser power of about 5-10W in a few meters of fiber. To achieve higher powers, techniques to increase the threshold for SBS must be used and they rely on decreasing the intensity by using large mode area (LMA) fibers and on decreasing the effective interaction length by disrupting the coherence of the acoustic wave while maintaining the coherence length of the optical wave. Both of these approaches have been investigated with good success in the last decade. Disruption of the acoustic interaction length has been accomplished by introducing a longitudinal temperature gradient  \textcolor{red}{SBS Temp grad Ref} and by introducing radial discontinuities in the material doping thus giving rise to different acoustic modes interfering destructively with each other \textcolor{red}{Reference}. For example using a LMA fiber, 12m long and with a core diameter of 30um, a SBS threshold of 40W was increased to greater than 150W by using the same LMA but with a graded Ge/Al co-doped core designed to disrupt the acoustic properties of the fiber \cite{Li2007}. In subsequent work the SBS threshold was increased to 500W \textcolor{red}{REFERENCE} and most numerical models predicted that one kW should be attainable from a narrow band, single mode fiber. In practice this was not achieved because of the onset of very strong mode instabilities, resulting in a rapid degradation of the beam quality at powers above 500W \textcolor{red}{REFERENCE} to be discussed below. 

\paragraph{Single Frequency Fiber Lasers for GW Detectors}
High power fiber lasers for gravitational wave detectors have been investigated and may possibly be used later on in the advanced VIRGO detector \textcolor{red}{VIRGO Fiber laser Ref}. The fibers used were commercially available LMA fibers or photonic crystal rods and low noise amplification at $1 \nu m$ were obtained up to a power of 100W. No degradation or increased phase noise was measured \textcolor{red}{Nary Man et al 2010 Ref}. However, current indications are that when left on continually, the power output decreases due to photo-darkening in the fiber. This has been investigated by others and may be due to very small traces of other rare earth element impurities. Thus traces of Thulium as small as parts per billion have been found to lead to photo-darkening, attributed from UV emission from excited state absorption in these impurities \textcolor{red}{Photo darkening Ref}. This photo-darkening can be prevented by operating at lower powers and there are some reports that the effect is not permanent. This will need to be resolved. One proposed design for advanced VIRGO uses two of these fiber amplifiers coherently combined in parallel to achieve the necessary power, but additional work on the characterization, lifetime and engineering of the fiber lasers remain to be done. In other preliminary work using a commercially available fiber laser amplifier to amplify the output of an NPRO to 50W for gravitational wave research at the ACIGA facility, spatial variations in the beam were observed, possibly due to mode instabilities \textcolor{red}{Mode instabilites Ref}. However, these problems may be surmountable and fiber lasers may well be developed for third generation GW detectors as described below. 

\subsection{Lasers for Third generation and Beyond}
The design discussed here will require higher powers \textcolor{red}{PowerSection} and longer wavelengths \textcolor{red}{WavelengthSection}.  Thus laser designs in the 200W-400W range are of interest, as are wavelengths in the \GwincVal{Blue.Laser.Wavelength_nm}\,nm range which are well above the band-gap of silicon, \textcolor{red}{2PhotonAbsorptionSection} which is the material selected for the test masses in Voyager (\textcolor{red}{SiliconSection}. In what follows we provide a glimpse of what today appears to be attractive possibilities for future detectors.

\subsubsection{Fiber Laser Amplifier}
As discussed above, current limitations on single frequency, low noise fiber amplifiers appear to be the onset of SBS close to 100W. Further detailed studies of phase noise in LAM fiber amplifiers need to be undertaken while incorporating techniques to suppress SBS and transverse mode instabilities. Furthermore fiber laser amplifiers using different materials and dopants need to be investigated to assess the available wavelength range of these devices and the prevention of photo-darkening and other possible non-linear effects.

At the time of writing 100 W was the maximum power that had been achieved in a polarization maintaining fiber at a single frequency \textcolor{red}{SingleFreqPowerReference} and at low noise consistent with gravitational wave detectors, but with insufficient long term reliability \textcolor{red}{ManBrilletReference}.  More recent works reporting higher powers have not usually reported simultaneous achievements of single frequency, single mode and low phase noise required for our purpose. Nonetheless, considerable advances have been made in high power fiber lasers in general (\textcolor{red}{Review Jauregui 2103 Ref} and for fibers potentially useful for gravitational wave detectors. Thus single frequency SBS free, polarization maintaining fiber amplifiers have been developed to beyond 400W \textcolor{red}{Jeung 2007 Ref} and acoustically segmented photonic fibers to nearly 500W \textcolor{red}{Robin 2011 Ref}, but with imperfect beam quality, whereas 203W was estimated to be in \(TEM_{00}\)  \textcolor{red}{Karow 2012 Ref} but with no phase noise measurements. 

In all cases, either the onset of SBS or transverse mode instabilities limit the maximum power attainable.  The mode instabilities were observed to occur with a distinct threshold at about 275W for a LAM, 63 micron core fiber amplifier \textcolor{red}{Eidam 2011 Ref} and has been analyzed by many authors since then. Thus \textcolor{red}{Smith 2011 Ref}\textcolor{red}{Ward 2012 Ref} analyzed the thermal origin of the instabilities and traced them to the creation of a thermo-optic grating created by the interference of the fundamental and a higher mode in the fiber, allowed by the large diameter. Much progress has been made in improving the understanding of the origin of the mode instabilities \textcolor{red}{Jauregui 2012 Ref} and increasing the power threshold for the onset of the instability, concentrating primarily on reducing the gain available to the higher order modes by more efficient gain saturation, choice of pump wavelengths, choice of fibers and fiber geometries. The theoretical understanding is not complete and much work on increasing the threshold for the mode instabilities is being done worldwide, both analytically and experimentally. However for our purpose it seems reasonable to assume that reliable fiber amplifiers can be made in the power regime required, but this needs to be demonstrated for single frequency and low noise.  Long term reliability and approaches to prevent possible photo-darkening also need to be studied. Due to the highly competitive market in fiber lasers, it is quite possible that progress on these topics have already been made, but not published in the open literature.

Fiber laser amplifiers are also attractive because of their long interaction lengths allowing efficient lasing using other dopants. Thus fiber lasers have been developed to emit at 1550nm using Er doping, and very efficient high power fiber lasers have been demonstrated using thulium at ~1900nm and holmium at ~2000nm. \textcolor{red}{Thalium doping Ref} \textcolor{red}{Holmium doping Ref}  These laser hosts have not yet been developed for single frequency low noise, and for use in gravitational wave detectors, reliable master oscillators must also be developed. NPROs using these dopants have been developed in YAG hosts (see below) but the resultant wavelengths are not necessarily suitable for use in glass fiber lasers.

Thus it appears that the use of high power fiber laser amplifiers for gravitational wave detection are promising, but will require research to combine the approaches for mitigating SBS and mode instabilities with the simultaneous requirements for reliable single frequency, polarized, low noise operation and/or make use of coherent combination of individual lower power devices.  Finally, the devices need to be optimized for the preferred wavelength.






==> ParametricInstabilities.tex <==
\subsection{Parametric Instabilities}

The optical cavities and the interferometer mirrors have high quality factors, which allow for highly amplified resonances in the system. The accidental overlap of the resonances can lead to parametric instabilities~\cite{}.

\begin{figure}
\includegraphics[width=\columnwidth]{figures/PI-Loop.pdf}
\caption{Feedback loop diagram of opto-mechanical parametric instabilities}
\label{fig:PI}
\end{figure}



==> Power_budget.tex <==
\label{s:PB}
words

==> QE_table.tex <==

\begin{table}
  \begin{center}
    \begin{tabular}{lccccccc}\\ \toprule
      &     & \multicolumn{2}{c}{$\lambda = 1064\,{\rm nm}$}
            & \multicolumn{2}{c}{$\lambda = 1550\,{\rm nm}$}
            & \multicolumn{2}{c}{$\lambda = 2000\,{\rm nm}$} \\
Manufacturer & P/N & R [A/W] & Q.E. & R [A/W] & Q.E. & R [A/W] & Q.E. \\ \midrule
Excelitas      & C30665 & 0.78 & 0.91 & 1.05 & 0.84 & N/A & N/A \\
Laser Components & IG17 & 0.72 & 0.84 & 1.07 & 0.86 & N/A & N/A \\
Laser Components & IG19 & 0.57 & 0.66 & 1.00 & 0.80 & N/A & N/A \\
Laser Components & IG22 & 0.60 & 0.70 & 1.07 & 0.86 & 1.30$\sim$1.40 & 0.81$\sim$0.87 \\
Laser Components & IG24 & 0.37 & 0.43 & 0.90 & 0.72 & 1.36 & 0.84 \\
Laser Components & IG26 & 0.55 & 0.64 & 0.90 & 0.72 & 1.40 & 0.87 \\
Hamamatsu        & G8605 & 0.67 & 0.78 & 0.95 & 0.76 & N/A & N/A \\
Hamamatsu        & G10899 & 0.74 & 0.86 & 1.0 & 0.80 & N/A & N/A \\
Hamamatsu        & G12180 & 0.60 & 0.70 & 1.1 & 0.88 & N/A & N/A \\
Hamamatsu        & G12183 & 0.35    & .0.41   & 1.05    & 0.84    & 1.24 & 0.77 \\
Thorlabs         & FGA21  & 0.57 & 0.66 & 1.03 & 0.82 & N/A & N/A \\ \bottomrule
\end{tabular}
\caption[QE of commercial InGaAs PDs]{Responsivity and quantum efficiencies of commercially available InGaAs photodiodes. Asterisk indicates without a window in front of the diode.}
\label{t:InGaAs}
\end{center}
\end{table}

==> Voyager_author_list.tex <==
% [AIDAN]: 31-AUG-2019:  Based on AUG-2017 IS author list.
\author{%
R.~X.~Adhikari$^{1}$,  %rana.adhikari
K.~Arai$^{1}$, 	%koji.arai
A.~F.~Brooks$^{1}$,  %aidan.brooks
C.~C.~Wipf$^{1}$,  %christopher.wipf
R.~Abbott$^{1}$,  %rich.abbott
T.~D.~Abbott$^{2}$,  %thomas.abbott
C.~Adams$^{3}$,  %carl.adams
V.~B.~Adya$^{4}$,  %vaishali.adya
A.~Ananyeva$^{1}$,  %alena.ananyeva
S.~Appert$^{1}$,  %stephen.appert
S.~M.~Aston$^{3}$,  %stuart.aston
C.~Austin$^{2}$, 	%corey.austin
S.~W.~Ballmer$^{5}$,  %stefan.ballmer
D.~Barker$^{6}$,  %david.barker
B.~Barr$^{7}$,  %bryan.barr
L.~Barsotti$^{8}$,  %lisa.barsotti
J.~Bartlett$^{6}$,  %jeffrey.bartlett
I.~Bartos$^{9}$,  %imre.bartos
J.~C.~Batch$^{6}$,  %james.batch
A.~S.~Bell$^{7}$,  %angus.bell
J.~Betzwieser$^{3}$,  %joseph.betzwieser
G.~Billingsley$^{1}$,  %garilynn.billingsley
J.~Birch$^{3}$,  %jeremy.birch
S.~Biscans$^{8}$,  %sebastien.biscans
C.~Biwer$^{5}$,  %christopher.biwer
C.~D.~Blair$^{3}$,  %carl.blair
R.~M.~Blair$^{6}$,  %ryan.blair
R.~Bork$^{1}$,  %rolf.bork
H.~Cao$^{10}$,  %huy-tuong.cao
G.~Ciani$^{9}$,  %giacomo.ciani
F.~Clara$^{6}$,  %filiberto.clara
S.~J.~Cooper$^{11}$,  %sam.cooper
P.~Corban$^{3}$, %paul.corban
S.~T.~Countryman$^{12}$,  %stefan.countryman
P.~B.~Covas$^{13}$,  %pep.covas
M.~J.~Cowart$^{3}$,  %matthew.cowart
D.~C.~Coyne$^{1}$,  %dennis.coyne
A.~Cumming$^{7}$,  %alan.cumming
L.~Cunningham$^{7}$,  %liam.cunningham
K.~Danzmann$^{14,4}$,  %karsten.danzmann
C.~F.~Da~Silva~Costa$^{9}$, %filipe.dasilva
E.~J.~Daw$^{15}$,  %edward.daw
D.~DeBra$^{16}$,  %dan.debra
R.~T.~DeRosa$^{3}$,  %ryan.derosa
R.~DeSalvo$^{17}$,  %riccardo.desalvo
K.~L.~Dooley$^{18}$,  %katherine.dooley
S.~Doravari$^{4}$,  %suresh.doravari
J.~C.~Driggers$^{6}$,  %jenne.driggers
S.~E.~Dwyer$^{6}$,  %sheila.dwyer
T.~B.~Edo$^{15}$,  %tega.edo
A.~Effler$^{3}$,  %anamaria.effler
T.~Etzel$^{1}$, %todd.etzel
M.~Evans$^{8}$,  %matthew.evans
T.~M.~Evans$^{3}$,  %tom.evans
M.~Factourovich$^{12}$,  %maxim.factourovich
H.~Fair$^{5}$, %hannah.fair
A.~Fern\'andez~Galiana$^{8}$, 	%alvaro.fernandez-galiana
E.~C.~Ferreira$^{19}$,  %elvis.ferreira
R.~P.~Fisher$^{5}$, % 	ryan.fisher
H.~Fong$^{20}$,  %heather.fong
R.~Frey$^{21}$,  %raymond.frey
P.~Fritschel$^{8}$,  %peter.fritschel
V.~V.~Frolov$^{3}$,  %valery.frolov
P.~Fulda$^{9}$,  %paul.fulda
M.~Fyffe$^{3}$,  %michael.fyffe
B.~Gateley$^{6}$, %bubba.gateley
J.~A.~Giaime$^{2,3}$,  %joe.giaime
K.~D.~Giardina$^{3}$,  %dwayne.giardina
E.~Goetz$^{6}$,  %evan.goetz
R.~Goetz$^{9}$, %ryan.goetz
S.~Gras$^{8}$,  %slawomir.gras
C.~Gray$^{6}$,  %corey.gray
H.~Grote$^{4}$, %hartmut.grote
K.~E.~Gushwa$^{1}$,  %kaitlin.gushwa
E.~K.~Gustafson$^{1}$,  %eric.gustafson
R.~Gustafson$^{22}$,  %dick.gustafson
E.~D.~Hall$^{8}$,  %evan.hall
G.~Hammond$^{7}$,  %giles.hammond
J.~Hanks$^{6}$,  %jonathan.hanks
J.~Hanson$^{3}$,  %joe.hanson
T.~Hardwick$^{2}$, %terra.hardwick
G.~M.~Harry$^{23}$,  %gregg.harry
M.~C.~Heintze$^{3}$,  %matthew.heintze
A.~W.~Heptonstall$^{1}$,  %alastair.heptonstall
J.~Hough$^{7}$,  %james.hough
K.~Izumi$^{6}$,  %kiwamu.izumi
R.~Jones$^{7}$,  %russell.jones
S.~Kandhasamy$^{3}$, %shivaraj.kandhasamy
S.~Karki$^{21}$,  %sudarshan.karki
M.~Kasprzack$^{2}$, %marie.kasprzack
S.~Kaufer$^{14}$, %steffen.kaufer
K.~Kawabe$^{6}$,  %keita.kawabe
R.~Kennedy$^{15}$,  %ross.kennedy
N.~Kijbunchoo$^{24}$,  %nutsinee.kijbunchoo
W.~Kim$^{10}$,  %won.kim
E.~J.~King$^{10}$, %eleanor.king
P.~J.~King$^{6}$,  %peter.king
J.~S.~Kissel$^{6}$,  %jeffrey.kissel
W.~Z.~Korth$^{1}$, %william.korth
G.~Kuehn$^{4}$, %gerrit.kuehn
M.~Landry$^{6}$,  %michael.landry
B.~Lantz$^{16}$,  %brian.lantz
M.~Laxen$^{3}$, %michael.laxen
J.~Liu$^{25}$,  %liu.jian
N.~A.~Lockerbie$^{26}$,  %nick.lockerbie
M.~Lormand$^{3}$,  %marc.lormand
A.~P.~Lundgren$^{4}$,  %andrew.lundgren
M.~MacInnis$^{8}$,  %myron.macinnis
D.~M.~Macleod$^{27}$,  %duncan.macleod
S.~M\'arka$^{12}$,  %szabolcs.marka
Z.~M\'arka$^{12}$,  %zsuzsanna.marka
A.~S.~Markosyan$^{16}$,  %ashot.markosyan
E.~Maros$^{1}$, %ed.maros
P.~Marsh$^{28}$, %paul.marsh
I.~W.~Martin$^{7}$, %ian.martin
D.~V.~Martynov$^{8}$,  %denis.martynov
K.~Mason$^{8}$,  %ken.mason
T.~J.~Massinger$^{1}$, %thomas.massinger
F.~Matichard$^{1,8}$,  %fabrice.matichard
N.~Mavalvala$^{8}$,  %nergis.mavalvala
R.~McCarthy$^{6}$,  %richard.mccarthy
D.~E.~McClelland$^{24}$,  %david.mcclelland
S.~McCormick$^{3}$,  %scott.mccormick
L.~McCuller$^{8}$,  %lee.mcculler
G.~McIntyre$^{1}$,  %gary.mcintyre
J.~McIver$^{1}$,  %jessica.mciver
T.~McRae$^{24}$,  %terry.mcrae
G.~Mendell$^{6}$,  %gregory.mendell
E.~L.~Merilh$^{6}$,  %edmond.merilh
P.~M.~Meyers$^{29}$, %patrick.meyers
J.~Miller$^{8}$, 	%john.miller
R.~Mittleman$^{8}$,  %richard.mittleman
K.~Mogushi$^{18}$,  %kentaro.mogushi
D.~Moraru$^{6}$,  %dan.moraru
G.~Moreno$^{6}$,  %gerardo.moreno
G.~Mueller$^{9}$,  %guido.mueller
N.~Mukund$^{30}$,  %nikhil.mukund
A.~Mullavey$^{3}$,  %adam.mullavey
J.~Munch$^{10}$,  %jesper.munch
T.~J.~N.~Nelson$^{3}$,  %timothy.nelson
P.~Nguyen$^{21}$, %philippe.nguyen
L.~K.~Nuttall$^{27}$,  %laura.nuttall
J.~Oberling$^{6}$,  %jason.oberling
M.~Oliver$^{13}$,  %miquel.oliver
P.~Oppermann$^{4}$,  %patrick.oppermann
Richard~J.~Oram$^{3}$,  %richard.oram
B.~O'Reilly$^{3}$,  %brian.oreilly
D.~J.~Ottaway$^{10}$,  %david.ottaway
H.~Overmier$^{3}$,  %harry.overmier
J.~R.~Palamos$^{21}$,  %jordan.palamos
W.~Parker$^{3}$,  %william.parker
A.~Pele$^{3}$,  %arnaud.pele
S.~Penn$^{31}$, %steven.penn
C.~J.~Perez$^{6}$,  %carlos.perez
M.~Phelps$^{7}$,  %margot.phelps
V.~Pierro$^{32}$, %vincenzo.pierro
I.~Pinto$^{32}$, %innocenzo.pinto
M.~Principe$^{32}$,  %maria.principe
L.~G.~Prokhorov$^{33}$, %leonid.prokhorov
O.~Puncken$^{4}$,  %oliver.puncken
V.~Quetschke$^{34}$,  %volker.quetschke
E.~A.~Quintero$^{1}$,  %eric.quintero
H.~Radkins$^{6}$,  %hugh.radkins
P.~Raffai$^{35}$, %peter.raffai
K.~E.~Ramirez$^{34}$,  %karla.ramirez
S.~Reid$^{36}$,  %stuart.reid
D.~H.~Reitze$^{1,9}$,  %david.reitze
N.~A.~Robertson$^{1,7}$,  %norna.robertson
J.~G.~Rollins$^{1}$,  %jameson.rollins
V.~J.~Roma$^{21}$,  %vincent.roma
C.~L.~Romel$^{6}$,  %chandra.romel
J.~H.~Romie$^{3}$,  %janeen.romie
M.~P.~Ross$^{37}$,  %michael.ross
S.~Rowan$^{7}$,  %sheila.rowan
K.~Ryan$^{6}$,  %kyle.ryan
T.~Sadecki$^{6}$,  %travis.sadecki
E.~J.~Sanchez$^{1}$,  %eduardo.sanchez
L.~E.~Sanchez$^{1}$,  %luis.sanchez
V.~Sandberg$^{6}$,  %vernon.sandberg
R.~L.~Savage$^{6}$,  %richard.savage
R.~M.~S.~Schofield$^{21}$,  %robert.schofield
D.~Sellers$^{3}$,  %danny.sellers
D.~A.~Shaddock$^{24}$,  %daniel.shaddock
T.~J.~Shaffer$^{6}$,  %thomas.shaffer
B.~Shapiro$^{16}$,  %brett.shapiro
D.~H.~Shoemaker$^{8}$,  %david.shoemaker
D.~Sigg$^{6}$,  %daniel.sigg
B.~J.~J.~Slagmolen$^{24}$,  %bram.slagmolen
B.~Smith$^{3}$,  %bryan.smith
J.~R.~Smith$^{38}$,  %joshua.smith
B.~Sorazu$^{7}$,  %borja.sorazu
A.~P.~Spencer$^{7}$,  %andrew.spencer
A.~Staley$^{12}$,  %alexan.staley
K.~A.~Strain$^{7}$,  %ken.strain
D.~B.~Tanner$^{9}$, %david.tanner
R.~Taylor$^{1}$,  %robert.taylor2
M.~Thomas$^{3}$,  %michael.thomas
P.~Thomas$^{6}$,  %patrick.thomas
K.~A.~Thorne$^{3}$,  %keith.thorne
E.~Thrane$^{39}$,  %eric.thrane
K.~Toland$^{7}$,  %karl.toland
C.~I.~Torrie$^{1}$,  %calum.torrie
G.~Traylor$^{3}$,  %gary.traylor
M.~Tse$^{8}$,  %maggie.tse
D.~Tuyenbayev$^{34}$,  %darkhan.tuyenbayev
G.~Vajente$^{1}$,  %gabriele.vajente
G.~Valdes$^{2}$, %guillermo.valdes
A.~A.~van~Veggel$^{7}$,  %marielle.vanveggel
A.~Vecchio$^{11}$,  %alberto.vecchio
P.~J.~Veitch$^{10}$,  %peter.veitch
K.~Venkateswara$^{37}$,  %krishna.venkateswara
T.~Vo$^{5}$,  %thomas.vo
C.~Vorvick$^{6}$,  %cheryl.vorvick
M.~Walker$^{38}$, %marissa.walker
R.~L.~Ward$^{24}$,  %robert.ward
J.~Warner$^{6}$,  %jim.warner
B.~Weaver$^{6}$,  %betsy.weaver
R.~Weiss$^{8}$,  %rainer.weiss
P.~We{\ss}els$^{4}$,  %peter.wessels
B.~Willke$^{14,4}$,  %benno.willke
J.~Worden$^{6}$,  %john.worden
H.~Yamamoto$^{1}$,  %hiro.yamamoto
C.~C.~Yancey$^{40}$,  %cregg.yancey
Hang~Yu$^{8}$,  %hang.yu
Haocun~Yu$^{8}$,  %haocun.yu
L.~Zhang$^{1}$,  %liyuan.zhang
M.~E.~Zucker$^{1,8}$,  %michael.zucker
and
J.~Zweizig$^{1}$%  %john.zweizig
\\
{(LSC Instrument Authors)}%
}%
\medskip
\address {$^{1}$LIGO, California Institute of Technology, Pasadena, CA 91125, USA }
\address {$^{2}$Louisiana State University, Baton Rouge, LA 70803, USA }
\address {$^{3}$LIGO Livingston Observatory, Livingston, LA 70754, USA }
\address {$^{4}$Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany }
\address {$^{5}$Syracuse University, Syracuse, NY 13244, USA }
\address {$^{6}$LIGO Hanford Observatory, Richland, WA 99352, USA }
\address {$^{7}$SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom }
\address {$^{8}$LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA }
\address {$^{9}$University of Florida, Gainesville, FL 32611, USA }
\address {$^{10}$OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia }
\address {$^{11}$University of Birmingham, Birmingham B15 2TT, United Kingdom }
\address {$^{12}$Columbia University, New York, NY 10027, USA }
\address {$^{13}$Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain }
\address {$^{14}$Leibniz Universit\"at Hannover, D-30167 Hannover, Germany }
\address {$^{15}$The University of Sheffield, Sheffield S10 2TN, United Kingdom }
\address {$^{16}$Stanford University, Stanford, CA 94305, USA }
\address {$^{17}$California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA }
\address {$^{18}$The University of Mississippi, University, MS 38677, USA }
\address {$^{19}$Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil }
\address {$^{20}$Canadian Institute for Theoretical Astrophysics, University of Toronto, Toronto, Ontario M5S 3H8, Canada }
\address {$^{21}$University of Oregon, Eugene, OR 97403, USA }
\address {$^{22}$University of Michigan, Ann Arbor, MI 48109, USA }
\address {$^{23}$American University, Washington, D.C. 20016, USA }
\address {$^{24}$OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia }
\address {$^{25}$OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia }
\address {$^{26}$SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom }
\address {$^{27}$Cardiff University, Cardiff CF24 3AA, United Kingdom }
\address {$^{28}$University of Washington Bothell, 18115 Campus Way NE, Bothell, WA 98011, USA }
\address {$^{29}$University of Minnesota, Minneapolis, MN 55455, USA }
\address {$^{30}$Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India }
\address {$^{31}$Hobart and William Smith Colleges, Geneva, NY 14456, USA }
\address {$^{32}$University of Sannio at Benevento, I-82100 Benevento, Italy and INFN, Sezione di Napoli, I-80100 Napoli, Italy }
\address {$^{33}$Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia }
\address {$^{34}$The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA }
\address {$^{35}$Institute of Physics, E\"otv\"os University, P\'azm\'any P. s. 1/A, Budapest 1117, Hungary }
\address {$^{36}$SUPA, University of the West of Scotland, Paisley PA1 2BE, United Kingdom }
\address {$^{37}$University of Washington, Seattle, WA 98195, USA }
\address {$^{38}$California State University Fullerton, Fullerton, CA 92831, USA }
\address {$^{39}$OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia }
\address {$^{40}$University of Maryland, College Park, MD 20742, USA }



==> WavefrontControl.tex <==
\label{s:AWC}

\textcolor{red}{(Another Aidan bit)}

\textbf{\R{This this a bit to much detail.  Perhaps a paragraph near the end where we list the technical issues which will have to be dealt with but are not important enough to be included in the paper.}} \\

\subsection{Thermal lensing}

Absorbed light in the coating and substrate of the test mass causes thermo-elastic distortion creating figure errors and thermal lensing that can degrade interferometer performance~\cite{TCSsomething}. For silica test masses, both effects are significant. Maintaining silicon test masses at the zero CTE point results in low thermo-elastic distortion, while thermal lensing in the substrate remains significant.

The defocusing power, $S$, (the reciprocal of the focal length) of the induced thermal lens may be approximated as
\begin{equation}
S = \frac{dn/dT}{\pi\kappa w^2}P_\mathrm{abs},
\end{equation}
where $dn/dT$ is the temperature coefficient of refractive index of the substrate, $\kappa$ is the thermal conductivity of the substrate, $w$ is the $1/e^2$ intensity radius of the laser beam, and $P_\mathrm{abs}$ is the absorbed optical power in the \textcolor{red}{test mass and coating}.

In the Advanced LIGO interferometers, thermal lens compensation is achieved using both radiative heating coils near the edge of the mirror surface, as well as by compensation optics (CPs) heated by a $CO_2$ laser projected in a pattern which creates a negative thermal lens. The heating coils mainly act to reduce surface deformations of the arm-cavity optics, while the heated compensation optics remove the thermal lens of the mirror substrate. Such a system would also be necessary for a cryogenic interferometer. 

In order to optimally control thermal lensing, we require: (a) a {\it test mass} in which absorbed interferometer power (and therefore thermal lensing) is minimized, (b) a {\it compensation plate} in which absorbed interferometer power (and therefore thermal lensing) is minimized, and (c) a compensation plate in which the thermal lensing response per Watt absorbed power is maximized. In this third point, we are implicitly referring to power absorbed in the CP from sources other than the interferometer.

Table \ref{tab:TCS} shows the amount of self-induced thermal lensing expected from absorbed interferometer power for the Advanced LIGO test mass, a cryogenic silicon test mass, a room-temperature fused silica compensation plate and a room-temperature silicon compensation plate.


\begin{table}
\centering
\begin{tabular}{ |c| c| c| c| c | }
  \hline
   & aLIGO & Si-TM & SiO$_2$-CP & Si-CP \\ 
  \hline \hline
  Temperature, T (K) & 300 & 123 & 300 & 300 \\ \hline
  Absorbed power, $P_\textrm{abs}$ (W) & 0.4 & 3 & 0.25 & xx \\ \hline
  Thermo-refractive coeff., $dn/dT$ (K$^{-1}$) & 8.6E-6 & 9.5E-5 & 8.6E-6 & 1.8E-4 \\ \hline
  Thermal conductivity, $\kappa$ (W/m.K) & 1.38 & 500 & 1.38 & 150\\ \hline
  Beam size, $w$ (cm) & 5.4 & \GwincVal{Blue.Optics.ITM.BeamRadius_cm} & \GwincVal{Blue.Optics.ITM.BeamRadius_cm} & 5.9 \\ \hline
   \hline
  Defocus, $S$ ($\upmu$D)  & 272 & 66 & 170 & xx \\
\hline
\end{tabular}
\caption{Total substrate lens self-induced by each optic.}
\label{tab:TCS}
\end{table}

A fused silica compensation plate produces three times as much self-induced thermal lensing as the test mass it is there to compensate. Although the total thermal lens to correct ($66$ $\mu$D + 170$\mu$D = 236 $\mu$D) is of the order of the aLIGO thermal lens (272 $\mu$D), this is still a sub-optimal starting point.

{\it Need a table here that shows the response of different materials to applied power. Shows that Si@300K is optimum CP material.}

%--------------------------------------
\subsubsection{Actuator configuration}

\begin{itemize}
\item Test masses? No
\item Compensation plates: Yes
\item Beam splitter: yes
\item Power/signal recycling core optics: yes times 2
\item input optics: yes x2
\item SRC to OMC: yes x 2
\item SQZ to FC: yes x 2
\item FC to IFO: yes x 2
\end{itemize}

\subsection{Static lens correction}

A future interferometer will require significant control over the mode-matching between the input mode cleaner, the interferometer (with its four internal cavities), the injected squeezed filed, the filter cavity and the output mode cleaner.

\subsection{Higher order modes and PI control}

Proposal to aid in PI control with AWC in the SRC.



%For Voyager a $CO_2$ laser projection system coupled with fused silica compensation optics (located in the power recycling cavity) can be used to compensate for thermal lensing in the test masses. There would need to be some modifications to the general design, however. In Advanced LIGO, the compensation optics also play the role of the reaction mass for test mass force actuation. This will not be possible in a cryogenic design because the heated compensation optic would radiate heat to the cryogenic test mass, requiring significant additional cooling power. Instead the reaction mass would be a cooled silicon optic, while a separate fused silica compensation optic would operate at room temperature. With these modifications, thermal lens compensation in the style of Advanced LIGO would be sufficient for a cryogenic interferometer.




==> overview.tex <==
t\label{s:overview}


% \textcolor{red}{I THINK THIS SECTION SHOULD STOP HERE AND THE TECHNICAL STUFF ABOUT SENSITIVITY TO TEMPERASTURE VARIATION SHOULD BE MOVED TO A SECTION ON TECHNICAL PROBLEMS. PERHAPS IN AN APPENDIX.}

% Show noise projection (GWINC).

% The tolerance of the test mass temperature around the silicon CTE zero
% crossing is most likely to be dependent on the substrate thermoelastic noise.
% Figure~\ref{fig:BlueGWINCtemp_tolerance} plots estimates of this noise
% contribution for various temperatures. These estimates suggest the test
% mass temperature tolerance should at most be $\pm$4\,K around 123\,K.
% The plot considers the temperature dependence of the substrate CTE,
% specific heat, thermal conductivity, refractive index, and dn/dT over
% the temperature range. No temperature dependence of the mechanical
% loss is included.

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figures/BlueBird5_SubTE_vs_Temp.pdf}
%   \caption{Estimate of the silicon substrate thermoelastic noise as a
%     function of temperature. These curves were generated by updating
%     the temperature, substrate CTE, specific heat, thermal conductivity,
%     refractive index, and dn/dT over the temperature range. No
%     mechanical loss parameters were updated.}
%   \label{fig:BlueGWINCtemp_tolerance}
% \end{figure}

